From Traces To Proofs: Proving Concurrent Program Safe

Nondeterminism in scheduling is the cardinal reason for difficulty in proving correctness of concurrent programs. A powerful proof strategy was recently proposed [6] to show the correctness of such programs. The approach captured data-flow dependencies among the instructions of an interleaved and error-free execution of threads. These data-flow dependencies were represented by an inductive data-flow graph (iDFG), which, in a nutshell, denotes a set of executions of the concurrent program that gave rise to the discovered data-flow dependencies. The iDFGs were further transformed in to alternative finite automatons (AFAs) in order to utilize efficient automata-theoretic tools to solve the problem. In this paper, we give a novel and efficient algorithm to directly construct AFAs that capture the data-flow dependencies in a concurrent program execution. We implemented the algorithm in a tool called ProofTraPar to prove the correctness of finite state cyclic programs under the sequentially consistent memory model. Our results are encouranging and compare favorably to existing state-of-the-art tools.

==> petexpvert.tex <==
\newcommand{\stepone}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\fexstate{s1};
\setinitnode{s1};
\end{tikzpicture}
}

\newcommand{\steptwo}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\fexstate{s1};
\fexstate{s2};
\setinitnode{s1};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\end{tikzpicture}
}

\newcommand{\stepthree}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\small{\true}$};
\fexstate{s1};
\fexstate{s2};
\fexstate{s3};
\setinitnode{s1};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\end{tikzpicture}
}


\newcommand{\stepfour}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\small{\true}$};
\fexstate{s1};
\fexstate{s2};
\fexstate{s3};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\draw [->, loop right=-1pt] (s3) to node [above] {$r$} (s3) ;
\end{tikzpicture}
}

\newcommand{\stepfive}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\begin{array}{l}flag_1=0\\\|turn=2\end{array}$};
\node[existsnode, above left = of s3, label=left:$s_4$ ] (s4) {$flag_1=0$};
\node[existsnode, above right = of s3, label=left:$s_5$ ] (s5) {$turn=2$};
\setinitnode{s1};
\fexstate{s1};
\fexstate{s2};
\fallstate{s3};
\fexstate{s4};
\fexstate{s5};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\draw [->, loop right=-1pt] (s3) to node [above] {$r$} (s3) ;
\draw [->] (s3) to node [right] {$P$} (s4) ;
\draw [->] (s3) to node [right] {$P$} (s5) ;
\end{tikzpicture}
}

\newcommand{\stepsix}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\begin{array}{l}flag_1=0\\\|turn=2\end{array}$};
\node[existsnode, above left = of s3, label=left:$s_4$ ] (s4) {$flag_1=0$};
\node[existsnode, above right = of s3, label=left:$s_5$ ] (s5) {$turn=2$};
\fexstate{s1};
\fexstate{s2};
\fallstate{s3};
\fexstate{s4};
\fexstate{s5};
\setinitnode{s1};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\draw [->, loop right=-1pt] (s3) to node [above] {$r$} (s3) ;
\draw [->] (s3) to node [right] {$P$} (s4) ;
\draw [->] (s3) to node [right] {$P$} (s5) ;
\draw [->, loop right=-1pt] (s4) to node [above] {$p,q$} (s4) ;
\end{tikzpicture}
}

\newcommand{\stepseven}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\begin{array}{l}flag_1=0\\\|turn=2\end{array}$};
\node[existsnode, above left = of s3, label=left:$s_4$ ] (s4) {$flag_1=0$};
\node[existsnode, above right = of s3, label=left:$s_5$ ] (s5) {$turn=2$};
\node[finalexistsnode, above = of s5, label=left:$s_6$ ] (s6) {$\false$};
\fexstate{s1};
\fexstate{s2};
\fallstate{s3};
\fexstate{s4};
\fexstate{s4};
\fexstate{s6};

\setinitnode{s1};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\draw [->, loop right=-1pt] (s3) to node [above] {$r$} (s3) ;
\draw [->] (s3) to node [right] {$P$} (s4) ;
\draw [->] (s3) to node [right] {$P$} (s5) ;
\draw [->, loop right=-1pt] (s4) to node [above] {$p,q$} (s4) ;
\draw [->] (s5) to node [right] {$q$} (s6) ;
\draw [->, loop right=-1pt] (s6) to node [above] {$p,a,b,A$} (s6) ;
\end{tikzpicture}
}

\newcommand{\stepeight}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\begin{array}{l}flag_1=0\\\|turn=2\end{array}$};
\node[existsnode, above left = of s3, label=left:$s_4$ ] (s4) {$\begin{array}{l}flag_1=0 \land\\ (flag_2=0\\\|turn=1)\end{array}$};
\node[existsnode, above right = of s3, label=left:$s_5$ ] (s5) {$turn=2$};
\node[finalexistsnode, above = of s5, label=left:$s_6$ ] (s6) {$\false$};
\node[existsnode, above left = of s4, label=left:$s_7$ ] (s7) {$flag_1=0$};
\node[existsnode, above =of s4, label=left:$s_8$ ] (s8) {$\begin{array}{l}flag_2=0\\ \|turn=1\end{array}$};
\node[finalexistsnode, above left=of s8, label=left:$s_9$ ] (s9) {$flag_2=0$};
\node[existsnode, above right=of s8, label=left:$s_{10}$ ] (s10) {$turn=1$};
\fexstate{s1};
\fexstate{s2};
\fallstate{s3};
\fallstate{s4};
\fexstate{s5};
\fexstate{s6};
\fexstate{s7};
\fallstate{s8};
\fexstate{s9};
\fexstate{s10};

\setinitnode{s1};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\draw [->, loop right=-1pt] (s3) to node [above] {$r$} (s3) ;
\draw [->] (s3) to node [right] {$P$} (s4) ;
\draw [->] (s3) to node [right] {$P$} (s5) ;
\draw [->, loop right=-1pt] (s4) to node [above] {$p,q$} (s4) ;
\draw [->] (s5) to node [right] {$q$} (s6) ;
\draw [->] (s4) to node [right] {$A$} (s7) ;
\draw [->] (s4) to node [right] {$A$} (s8) ;
\draw [->] (s8) to node [right] {$\epsilon$} (s9) ;
\draw [->] (s8) to node [right] {$\epsilon$} (s10) ;
\draw [->, loop right=-1pt] (s9) to node [above] {$a,b$} (s9) ;
\draw [->, loop right=-1pt] (s6) to node [above] {$p,a,b,A$} (s6) ;
\end{tikzpicture}
}

\newcommand{\stepnine}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\begin{array}{l}flag_1=0\\\|turn=2\end{array}$};
\node[existsnode, above left = of s3, label=left:$s_4$ ] (s4) {$\begin{array}{l}flag_1=0 \land\\ (flag_2=0\\\|turn=1)\end{array}$};
\node[existsnode, above right = of s3, label=left:$s_5$ ] (s5) {$turn=2$};
\node[finalexistsnode, above = of s5, label=left:$s_6$ ] (s6) {$\false$};
\node[existsnode, above left = of s4, label=left:$s_7$ ] (s7) {$flag_1=0$};
\node[existsnode, above =of s4, label=left:$s_8$ ] (s8) {$\begin{array}{l}flag_2=0\\ \|turn=1\end{array}$};
\node[finalexistsnode, above left=of s8, label=left:$s_9$ ] (s9) {$flag_2=0$};
\node[existsnode, above right=of s8, label=left:$s_{10}$ ] (s10) {$turn=1$};
\node[finalexistsnode, above =of s10, label=left:$s_{11}$ ] (s11) {$\false$};
\fexstate{s1};
\fexstate{s2};
\fallstate{s3};
\fallstate{s4};
\fexstate{s5};
\fexstate{s6};
\fexstate{s7};
\fallstate{s8};
\fexstate{s9};
\fexstate{s10};
\fexstate{s11};
\setinitnode{s1};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\draw [->, loop right=-1pt] (s3) to node [above] {$r$} (s3) ;
\draw [->] (s3) to node [right] {$P$} (s4) ;
\draw [->] (s3) to node [right] {$P$} (s5) ;
\draw [->, loop right=-1pt] (s4) to node [above] {$p,q$} (s4) ;
\draw [->] (s5) to node [right] {$q$} (s6) ;
\draw [->] (s4) to node [right] {$A$} (s7) ;
\draw [->] (s4) to node [right] {$A$} (s8) ;
\draw [->] (s8) to node [right] {$\epsilon$} (s9) ;
\draw [->] (s8) to node [right] {$\epsilon$} (s10) ;
\draw [->] (s10) to node [right] {$b$} (s11) ;
\draw [->, loop right=-1pt] (s9) to node [above] {$a,b$} (s9) ;
\draw [->, loop right=-1pt] (s11) to node [above] {$a$} (s11) ;
\draw [->, loop right=-1pt] (s6) to node [above] {$p,a,b,A$} (s6) ;
\end{tikzpicture}
}

\newcommand{\stepten}{
\begin{tikzpicture}
\node[existsnode, label=below:$s_1$ ] (s1) {$\small{\neg (\ell_2=2)}$};
\node[existsnode, above= of s1, label=left:$s_2$ ] (s2) {$\small{\neg (cs=2)}$};
\node[existsnode, above= of s2, label=left:$s_3$ ] (s3) {$\begin{array}{l}flag_1=0\\\|turn=2\end{array}$};
\node[existsnode, above left = of s3, label=left:$s_4$ ] (s4) {$\begin{array}{l}flag_1=0 \land\\ (flag_2=0\\\|turn=1)\end{array}$};
\node[existsnode, above right = of s3, label=left:$s_5$ ] (s5) {$turn=2$};
\node[finalexistsnode, above = of s5, label=left:$s_6$ ] (s6) {$\false$};
\node[existsnode, above left = of s4, label=left:$s_7$ ] (s7) {$flag_1=0$};
\node[existsnode, above =of s4, label=left:$s_8$ ] (s8) {$\begin{array}{l}flag_2=0\\ \|turn=1\end{array}$};
\node[finalexistsnode, above left=of s8, label=left:$s_9$ ] (s9) {$flag_2=0$};
\node[existsnode, above right=of s8, label=left:$s_{10}$ ] (s10) {$turn=1$};
\node[finalexistsnode, above =of s10, label=left:$s_{11}$ ] (s11) {$\false$};
\node[finalexistsnode, above left =of s7, label=left:$s_{12}$ ] (s12) {$\false$};
\fexstate{s1};
\fexstate{s2};
\fallstate{s3};
\fallstate{s4};
\fexstate{s5};
\fexstate{s6};
\fexstate{s7};
\fallstate{s8};
\fexstate{s9};
\fexstate{s10};
\fexstate{s11};
\fexstate{s12};
\setinitnode{s1};
\draw [->] (s1) to node [right] {$s$} (s2) ;
\draw [->] (s2) to node [right] {$c$} (s3) ;
\draw [->, loop right=-1pt] (s3) to node [above] {$r$} (s3) ;
\draw [->] (s3) to node [right] {$P$} (s4) ;
\draw [->] (s3) to node [right] {$P$} (s5) ;
\draw [->, loop right=-1pt] (s4) to node [above] {$p,q$} (s4) ;
\draw [->] (s5) to node [right] {$q$} (s6) ;
\draw [->] (s4) to node [right] {$A$} (s7) ;
\draw [->] (s4) to node [right] {$A$} (s8) ;
\draw [->] (s8) to node [right] {$\epsilon$} (s9) ;
\draw [->] (s8) to node [right] {$\epsilon$} (s10) ;
\draw [->] (s10) to node [right] {$b$} (s11) ;
\draw [->] (s7) to node [right] {$a$} (s12) ;
\draw [->, loop right=-1pt] (s9) to node [above] {$a,b$} (s9) ;
\draw [->, loop left=-1pt] (s7) to node [above] {$b$} (s7) ;
\draw [->, loop right=-1pt] (s11) to node [above] {$a$} (s11) ;
\draw [->, loop right=-1pt] (s6) to node [above] {$p,a,b,A$} (s6) ;
\end{tikzpicture}
}
